Single Image Super-Resolution based on Wiener Filter in Similarity Domain

Single image super resolution (SISR) is an ill-posed problem aiming at estimating a plausible high resolution (HR) image from a single low resolution (LR) image. Current state-of-the-art SISR methods are patch-based. They use either external data or internal self-similarity to learn a prior for a HR image. External data based methods utilize large number of patches from the training data, while self-similarity based approaches leverage one or more similar patches from the input image. In this paper we propose a self-similarity based approach that is able to use large groups of similar patches extracted from the input image to solve the SISR problem. We introduce a novel prior leading to collaborative filtering of patch groups in 1D similarity domain and couple it with an iterative back-projection framework. The performance of the proposed algorithm is evaluated on a number of SISR benchmark datasets. Without using any external data, the proposed approach outperforms the current non-CNN based methods on the tested datasets for various scaling factors. On certain datasets, the gain is over 1 dB, when compared to the recent method A+. For high sampling rate (x4) the proposed method performs similarly to very recent state-of-the-art deep convolutional network based approaches.

==> table/stack_size_psnr.tex <==
% This code assumes the following pgfplotstable keys:
% colsep=comma

% The table with the data to show.
\pgfplotstableread[header=has colnames]{data/stack_size_psnr.csv}\thetable

\pgfplotstabletypeset[
	create on use/names/.style={
		create col/set list={Baby,Bird,Butterfly,Head,Woman,Average},
	},
	columns/names/.style={
		string type,
		column type={l},
		column name={},
	},
	every head row/.style={
		before row={%
			\toprule%
			&
			\multicolumn{6}{c}{Stack Size}\\
		},
		after row=\midrule,
	},
	every nth row={5}{before row=\midrule},
	columns/.add={names,2,4,8,16,32*,64},
]{\thetable}


